Tidal Disruptions of Stars by Black Hole Remnants in Dense Star Clusters

In a dense stellar environment, such as the core of a globular cluster (GC), dynamical interactions with black holes (BHs) are expected to lead to a variety of astrophysical transients. Here we explore tidal disruption events (TDEs) of stars by stellar-mass BHs through collisions and close encounters. Using state-of-the-art $N$-body simulations, we show that these TDEs occur at significant rates throughout the evolution of typical GCs and we study how their relative rates relate to cluster parameters such mass and size. By incorporating a realistic cosmological model of GC formation, we predict a BH - main-sequence-star TDE rate of approximately $3\,\rm{Gpc}^{-3}\,\rm{yr}^{-1}$ in the local universe ($z<0.1$) and a cosmological rate that peaks at roughly $25\,\rm{Gpc}^{-3}\,\rm{yr}^{-1}$ for redshift 3. Furthermore, we show that the ejected mass associated with these TDEs could produce optical transients of luminosity $\sim 10^{41} - 10^{44}\rm\,erg\,s^{-1}$ with timescales of about a day to a month. These should be readily detectable by optical transient surveys such as the Zwicky Transient Facility. Finally, we comment briefly on BH - giant encounters and discuss how these events may contribute to the formation of BH - white-dwarf binaries.

==> deleted_WL.tex <==
 and hence  The
post-disruption gas has a spread of specific energy $-\eta_{\rm
  max}\epsT<\eps<\eta_{\rm max}\epsT$, where $\eta_{\rm max}\sim 1$ is
a dimensionless number that depends the details of the hydrodynamic disruption process (e.g. the star's internal structure) and
\begin{equation}
  \label{eq:2}
  \epsT/c^2 = \rg R_*/\rt^2 \simeq 4.6\times10^{-6}\, M_1^{1/3} m_*^{2/3}
  r_*^{-1}. 
\end{equation}
The bound gas corresponds to negative specific energy $\eps =
-\eta\epsT$ and $\eta\in(0, \eta_{\rm max}]$. The most tightly bound
part $\eta = \eta_{\rm mas}$ will fall back to the pericenter first
and then more gas with smaller $\eta$ (larger apocenter radii) will
fall back towards the BH. The specific angular momentum is roughly given by
% that of the pre-disruption star $\ell\simeq \sqrt{2\rp \rg} c$
\begin{equation}
  \label{eq:3}
  \ell = \rp c\sqrt{2\rg/\rp + 2\eps} = \rp c\sqrt{2\rg/\rp - 2\eta \epsT},
\end{equation}
and the eccentricity is
\begin{equation}
  \label{eq:4}
  e = \sqrt{1 + 2\eps\ell^2/\rg^2c^4}.
\end{equation}
As shown in the upper panel of Fig. \ref{fig:ecc}, the orbits of fallback gas are not highly eccentric for the case of a main-sequence star disrupted by a stellar mass BH. This is very different from TDEs by supermassive BHs where we have $1-e\sim
(M_*/M)^{1/3}\ll 1$. We see that a nearly circular accretion disk
forms quickly after the most tightly bound mass falls back to the
pericenter, at the circularization radius
\begin{equation}
  \label{eq:5}
  \rc = \ell^2/\rg c^2.
\end{equation}
From the right panel of Fig. \ref{fig:ecc}, we see that the
circularization radius is a weak function of $\eta$ and a good
approximation for $1\lesssim \beta\lesssim 3$ is to take $\rc \simeq 1.5\rp =
1.5\rt/\beta$.
\begin{figure}
  \centering
\includegraphics[width = 0.48\textwidth,
  height=0.25\textheight]{sBH_ecc.pdf}
\includegraphics[width = 0.48\textwidth,
  height=0.25\textheight]{sBH_rp_rc.pdf}
\caption{\textit{Top panel}: the eccentricity for different
  segments of the fallback gas (characterized by their specific
  energy). \textit{Bottom panel}: the pericenter radius $\rp$ and
  circularization radius $\rc$. For both panels, we take the BH mass
  $M = 10\msun$ and stellar mass $M_*=0.5\msun$. \note{[NOTE: when $\rp<R_*$, the BH directly plunges into the star. ]}
}\label{fig:ecc}
\end{figure}



If the wind is fully ionized, the Thomson scattering optical depth above $r$ is $\tau(r) \simeq \kappa_{\rm s}\rho \min(\vw t_{\rm vis}, r)$, where $\kappa_{\rm s}=0.34\rm\, cm^2\,g^{-1}$ is the Thomson scattering opacity and $\vw t_{\rm vis}$ is the typical radial thickness of the wind with similar mass loss rate (since the wind power varies on a viscous timescale $t_{\rm vis}$). Then, the photon trapping radius $\rtr$ is where the diffusion time $t_{\rm diff} = \tau (\rtr) \,\mr{min}(\vw t_{\rm vis}, r)/c$ equals to the dynamical time $t_{\rm dy} = r/\vw$,
which means
\begin{equation}
  \label{eq:16}
  \rtr \simeq \mr{min}\left[
{\kappa_{\rm s}\dot{M}_{\rm w}\over 4\pi c}, \left(\kappa_{\rm
    s} \dot{M}_{\rm w} \vw^2 t_{\rm vis}^2\over 4\pi c\right)^{1/3} 
\right]
\end{equation}
On the lower panel of Fig. \ref{fig:Trad}, we show the photon trapping radius (assuming fully ionized wind) and the hydrogen recombination radius (where the LTE temperature
drops to $\sim10^4\rm\,K$) both in units of
$\rd$.

\begin{figure}
  \centering
\includegraphics[width = 0.48\textwidth,
  height=0.25\textheight]{sBH_Trad.pdf}
\includegraphics[width = 0.48\textwidth,
  height=0.25\textheight]{sBH_rtr.pdf}
\caption{\textit{Top panel}: The radiation (and gas)
  temperature near radius $\rc$ as a function of the power-law index
 $s$. \textit{Bottom panel}: The photon trapping radius $\rtr$ in units
 of $\rc$ (red and blue curves) under the assumption that the gas
 stays fully ionized. The hydrogen recombination radius $\rrec$ in
 units of $\rc$ is shown in green and cyan (for different cases). When $\rrec<\rtr$,
 photons escape due to recombination before the wind reaches the
 trapping radius. For both panels, we take the efficiency of escaping
 power $\feps=0.5$, viscosity parameter $\alpha=0.1$, ISCO radius
  $\risco=6\rg$, and stellar mass $M_*=0.5\msun$.
}\label{fig:Trad}
\end{figure}

There are two possible cases, depending on whether
hydrogen recombination occurs before or after the wind reaches $\rtr$ given by eq. (\ref{eq:16}). Radiation escapes from the system at radius $\resc = \mr{min}(\rtr,
\rrec)$, where the recombination radius is defined as
$(\rrec/\rd)^{2/3} = T(\rd)/10^4\mr{\,K}$. Therefore, the escaping (observed) luminosity from the
system is given by
\begin{equation}
  \label{eq:17}
  L_{\rm obs} = 4\pi \resc^2 U(\resc) \vw = (L_{\rm d}/2)
  (\resc/\rd)^{-2/3},
\end{equation}
where $U(\resc)$ is given by eq. (\ref{eq:Urad}).
The escaping luminosity corresponding to the peak accretion rate (and peak disk luminosity) is shown in  Fig. \ref{fig:Lesc}, and we see that it is a sensitive function of the accretion rate powerlaw index $s$. For heavier wind mass loading, the escaping luminosity is strongly suppressed due to adiabatic loss (radiation pressure doing PdV work during the wind expansion). The color temperature of the escaping radiation\footnote{The thermalization radius is defined where the effective optical depth $\tau_*(r_{\rm th})\simeq \sqrt{\tau_{\rm abs}\tau}\simeq 1$ \note{[REF Rybicki and Lightman]}, where $\tau_{\rm abs}\simeq \kappa_{\rm abs}\rho\, \mr{min}(\vw t_{\rm vis}, r)$ is the absorption optical depth. In the case when $\rtr<r_{\rm th}<\rrec$, the color temperature predicted by our model is too high by a factor of $(r_{\rm th}/\rtr)^{2/3}$ but the bolometric luminosity is still correct.} is $T_{\rm obs} = \left[U(\resc) c/4\sigma_{\rm SB}\right]^{1/4}$.

Our treatment on the wind thermodynamics is based on the assumption that a stead-state wind is established quickly after the launching. This is appropriate if the wind expansion timescale $\resc/\vw$ is short compared to the viscous timescale $t_{\rm vis}$.

So far, we have assumed a steady-state wind.

After a viscous timescale $t_{\rm vis}$ (eq. \ref{eq:6}), the accretion rate drops with time as $\dot{M}(\rc)\propto [(t+t_{\rm vis})/t_{\rm vis}]^{-4/3}$
% \citep{1990ApJ...351...38C} 
and so the escaping luminosity is given by
eq. (\ref{eq:17}) according to the time-dependent accretion
rate. \note{[The viscouse spread of the disk is missing here. The viscous timescale evolves with time as well. ]} Also, before the wind reaches radius $\resc$, the lightcurve has
a rising period lasting for $\resc/\vw$, which is not captured here
(it can be included).

\begin{figure}
  \centering
\includegraphics[width = 0.48\textwidth,
  height=0.25\textheight]{sBH_Lesc1.pdf}
\includegraphics[width = 0.48\textwidth,
  height=0.25\textheight]{sBH_Lesc2.pdf}
\caption{\textit{Top panel}: The peak escaping luminosity as a
  function of the power-law index $s$ for $\alpha = 0.1$. \textit{Bottom panel}: The
  peak escaping luminosity for $\alpha=0.01$. For both
  panels, we take the efficiency of escaping power $\feps=0.5$, ISCO
  radius $\risco=6\rg$, and stellar mass $M_*=0.5\msun$.
}\label{fig:Lesc}
\end{figure}

\begin{figure}
  \centering
\includegraphics[width = 0.48\textwidth,
  height=0.25\textheight]{sBH_Lobs.pdf}
\includegraphics[width = 0.48\textwidth,
  height=0.25\textheight]{sBH_Tobs.pdf}
\caption{\textit{Top panel}: The bolometric lightcurves for
  $\alpha = 0.1$ (red) and $0.01$ (blue), and different accretion rate
  powerlaw indexes shown in the legend. \textit{Top panel}: The
  color temperature of the escaping radiation for $\alpha = 0.1$ (red)
  and $0.01$ (blue). For both panels, we take the efficiency of
  escaping power $\feps=0.5$, ISCO radius $\risco=6\rg$, and stellar
  mass $M_*=0.5\msun$.
}\label{fig:Lobs}
\end{figure}

If we take the case with $s=0.6$ and
$\alpha=0.1$, the peak luminosity is $\sim10^{43}\rm\,erg\,s^{-1}$
lasting for $\sim$a few days. 

% The left panel of Fig. \ref{fig:Ld} shows the total disk luminosity as a (very sensitive) function of the powerlaw index $s$, for different BH masses and impact parameters. We see that the total disk luminosity may vary by three orders of magnitude from the heaviest wind mass loss
% ($s\simeq 1$) to no wind ($s\simeq 0$). Our final results will be largely affected by this uncertainty.

% \begin{figure}
%   \centering
% \includegraphics[width = 0.48\textwidth,
%   height=0.25\textheight]{sBH_Ld.pdf}
% \includegraphics[width = 0.48\textwidth,
%   height=0.25\textheight]{sBH_vw.pdf}
% \caption{\textit{Top panel}: The total disk luminosity
%   (including kinetic and radiative power) as a function of the
%   accretion rate powerlaw index $s$. \textit{Bottom panel}: The
%   asymptotic wind velocity as a function of the powerlaw index
%   $s$. For both panels, we take the efficiency of escaping power
%   $\feps=0.5$, viscosity parameter $\alpha=0.1$, ISCO radius
%   $\risco=6\rg$, and stellar mass $M_*=0.5\msun$.
% }\label{fig:Ld}
% \end{figure}
